Global Prompt Cell: A Portable Control Module for Effective Prompt Tuning

As a novel approach to tuning pre-trained models, prompt tuning involves freezing the parameters in downstream tasks while inserting trainable embeddings into inputs in the first layer. However, previous methods have mainly focused on the initialization of prompt embeddings. The strategy of training and utilizing prompt embeddings in a reasonable way has become a limiting factor in the effectiveness of prompt tuning. To address this issue, we introduce the Global Prompt Cell (GPC), a portable control module for prompt tuning that selectively preserves prompt information across all encoder layers. Our experimental results demonstrate a 5.8% improvement on SuperGLUE datasets compared to vanilla prompt tuning.

==> content/discussion.tex <==
\section{Discussion}
To further investigate the effectiveness of our proposed Global Prompt Cell (GPC), we conducted additional experiments to compare the impact of the GPC model design versus the addition of trainable parameters to the vanilla prompt tuning model. Specifically, we wanted to verify that the improved performance of GPC was due to the novel model structure, rather than simply the addition of parameters.


While the prompt tuning inserts the initialized prompt into the input token embeddings before sending it to the first encoder layer and just updates the prompt by multi-layer encoders, GPC uses the remembering unit to process the pre-encoded prompt embeddings and the forgetting unit to process the post-encoded prompt embeddings between every two adjacent encoders. Furthermore, we discuss only using the inserted prompt in the first layer as history information, and compare the performance with GPC.

In the following formula, $P_t$ refers to the pre-encoded prompt embeddings of the $t$ th layer, while $P_t^*$ represents the post-encoded prompt embeddings of the $t$ th layer. $P_0$ is the randomly initialized prompt embeddings inserted to the input of first layer.

\paragraph{Direct Add Method}
The most direct method is to add the prompt embeddings in the first layer with the prompt embedding outputs in the other encoder layers, as Figure~\ref{v123} (a), which does not require any extra parameters.
\begin{equation}
 P_{t+1} = P_0 + P_{t}^{*} 
\end{equation}




\paragraph{Remembering Unit}
With a remembering unit, the prompt embeddings in the first layer are added to the post-encoded prompt after passing through the same remembering unit, as Figure~\ref{v123} (b). $W_P$ refers to the remembering unit used for all layers.
\begin{equation}
 P_{t+1} = W_{P}P_0 + P_{t}^{*}
\end{equation}



\paragraph{Multi Remembering Units}

The prompt embeddings in the first layer are added to the post-encoded prompt after passing through the layer-specific remembering units, as Figure~\ref{v123} (c), which involves most extra parameters. $W_P^t$ refers to the weight of the remembering unit of the $t$ th layer.

\begin{equation}
P_{t+1} = W_{P}^{t}P^0 + P_{t}^{*} 
\end{equation}

\begin{figure}[htbp]

\centering 
\includegraphics[width=1\columnwidth]{table/Figure/v1v2v3-line.pdf} 
\caption{The models that only use the inserted prompt in the first layer as history information.} 
\label{v123} 
\end{figure}

The experiment results in Table~\ref{discussion} show that adding the initial prompt to the post-encoded prompt would worsen the performance, so the improvement of results in our method does not come from the additional trainable parameters but the model structure design.


==> table/lab2-1_backpu.tex <==
% \usepackage{hhline}


\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\scalebox{0.85}{
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll clclc l clclc } 
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{5}{c}{BoolQ}                          & \multicolumn{1}{c}{} & \multicolumn{5}{c}{RTE}             \\ 
\cline{3-7}\cline{9-13}
                     &                      & PT            &  & Prompt-only &  & GPC    &                      & PT            &  & Prompt-only &  & GPC      \\ 
\midrule

BERT_{\ large}           &                      & 67.2 &  & 62.8        &  & \textbf{67.9}          &                      & 53.5          &  & 54.5        &  & \textbf{61.0}  \\
RoBERTa_{\ large}        &                      & 62.3          &  & 62.4        &  & \textbf{63.5} &                      & 58.8 &  & 54.2        &  & \textbf{59.4}           \\ 
\midrule
\midrule

\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{5}{c}{CB}    & \multicolumn{1}{c}{} & \multicolumn{5}{c}{COPA}               \\ 
\cline{3-7}\cline{9-13}
                     &                      & PT            &  & Prompt-only &  & GPC    &                      & PT            &  & Prompt-only &  & GPC  \\ 
\midrule

BERT_{\ large}  &     & 80.4 &  & 71.4          &  & \textbf{82.1}   
&        & 55.0            &  & 58.0          &  & \textbf{67.0}  \\
RoBERTa_{\ large}   &  & 71.4 &  & 69.6            &  & \textbf{73.2}  &                      & 63.0            &  & 62.0          &  & \textbf{66.0} \\ 





\midrule
\midrule




\multicolumn{1}{c}{}     & \multicolumn{1}{c}{} & \multicolumn{5}{c}{WiC}                           & \multicolumn{1}{c}{} & \multicolumn{5}{c}{WSC}                    \\ 
\cline{3-7}\cline{9-13}
                     &                      & PT            &  & Prompt-only &  & GPC    &                      & PT            &  & Prompt-only &  & GPC    \\ 
\midrule
BERT_{\ large}             &                      & 63.0            &  & 56.4        &  & \textbf{66.9} &                      & 64.4 &  & 64.4          &  & \textbf{65.4}   \\
RoBERTa_{\ large}     &              & 56.9          &  & 54.7        &  & \textbf{69.6} &                      & 64.4 &  & 63.5 &  & \textbf{65.4}          \\
\bottomrule
\end{tabular}
}}
\caption{Results on SuperGLUE development set. PT: Prompt tuning \citep{lester2021power}; Prompt-only: Prompt tuning with no verbalizer; GPC: Prompt tuning with Global Prompt Cell; \textbf{bold}: the best performance.}
\label{tab:my-table}
\end{table*}

==> table/lab2-2.tex <==
% \usepackage{hhline}

\begin{table*}[h]
\centering

%\renewcommand{\arraystretch}{1.1}
\scalebox{0.85}{
\resizebox{\textwidth}{!}{%
\begin{tabular}{l ccccc l ccccc} 
\toprule
              & \multicolumn{5}{c}{BooQ}                                         &  & \multicolumn{5}{c}{RTE}                                           \\ 
\cline{2-6}\cline{8-12}
              & PT             & DA   & RU   & MRU   & GPC     &  & PT             & DA   & RU   & MRU   & GPC         \\ 
\midrule
BERT    & 67.2  & 63.4 & 62.2 & 62.2 & \textbf{67.9}  &        
                & 53.5 & 54.5 & 52.7 & 53.1 & \textbf{61.0}  \\
RoBERTa & 62.3           & 62.2 & 62.2 & 62.2 & \textbf{63.5}  & &58.8  & 55.6 & 52.7 & 52.7 & \textbf{59.4}     \\ 

\midrule
\midrule

              &  \multicolumn{5}{c}{CB}          & & \multicolumn{5}{c}{COPA}       \\ 
\cline{2-6}\cline{8-12}
              & PT             & DA   & RU   & MRU   & GPC     &  & PT             & DA   & RU   & MRU   & GPC      \\ 
\midrule
BERT    
                & 80.4      & 76.8           & 50.0   & 59.0             & \textbf{82.1}  & & 55.0             & 62.0   & 62.0   & 61.0   & \textbf{67.0} \\
RoBERTa   & 71.4           & 62.5           & 50.0   & 50.0             & \textbf{73.2} & & 63.0             & 61.0   & 61.0   & 61.0   & \textbf{66.0}   \\ 


\midrule
\midrule


              &  \multicolumn{5}{c}{WiC}                                   &       & \multicolumn{5}{c}{WSC}                                                               \\ 
\cline{2-6}\cline{8-12}
              & PT             & DA   & RU   & MRU   & GPC    & & PT             & DA   & RU   & MRU   & GPC        \\ 
\midrule
BERT      & 63.0             & 52.2 & 54.2 & 50.8 & \textbf{66.9} & & 64.4           & 63.5           & 63.5 & 63.5           & \textbf{65.4}   \\
RoBERTa   & 56.9           & 53.9 & 50.0   & 51.1 & \textbf{69.6}  & & 64.4  & 64.4 & 63.5 & 64.4  & \textbf{65.4}            \\

\bottomrule
\end{tabular}}}
\caption{{Results of the ablation experiments. PT: Prompt-tuning~\citep{lester2021power}; DA: Direct Add Method; RU: Remembering Unit; MRU: Multi Remembering Units; GPC: Global Prompt Cell. \textbf{Bold}: the best performance.}}
\label{discussion}
\end{table*}
